GFGE: Unifying Explainable AI Methods through an Interpretation Framework

Explainable artificial intelligence (XAI) encompasses methods that draw on different sources of information and address different explanatory needs. A common framework is needed to describe how this information becomes evidence and is communicated as an explanation for a particular recipient. We propose the General Framework for Generating Explanations (GFGE), grounded in interpretative frameworks and the complementary activities of \emph{sense-reading} and \emph{sense-giving}. Its conceptual foundation is the Interpret/Explain Schema (IES), which connects an analyst's interpretation of system evidence, the communication of a selected account, and the recipient's interpretation of that account. GFGE operationalises this schema through five roles: data interpretation, model interpretation, output interpretation, optional post-hoc analysis, and aggregation. A role-typed operation graph records method-specific dependencies, while evidence records retain the sources, assumptions, and limitations of explanatory claims. The explanatory question, audience, and context guide the procedure. We instantiate GFGE for attribution, surrogate, counterfactual, concept and prototype, intrinsic rule, argumentation, and language-model methods. These instantiations show how intrinsic, post-hoc, and hybrid workflows can be represented through the same roles while preserving their distinct evidential requirements. GFGE provides a common basis for analysing explanation workflows, tracing communicated claims to their evidence, and identifying unresolved explanatory dependencies.

==> Figures/journal_style_v5.tex <==
% Publication artwork: native vector paths, embedded Helvetica, colour-independent labels.
\definecolor{gfInk}{HTML}{24343C}
\definecolor{gfRule}{HTML}{7A8990}
\definecolor{gfTeal}{HTML}{356B78}
\definecolor{gfTealFill}{HTML}{EFF5F6}
\definecolor{gfOchre}{HTML}{95662F}
\definecolor{gfOchreFill}{HTML}{FBF5EC}
\definecolor{gfSystemFill}{HTML}{F4F6F7}
\tikzset{
  gf base/.style={
    font=\fontfamily{phv}\selectfont\fontsize{8}{9.5}\selectfont,
    text=gfInk,>=Latex
  },
  gf box/.style={
    draw=gfRule,line width=0.65pt,rounded corners=1.5pt,
    fill=white,align=center,inner sep=5pt,outer sep=0pt
  },
  gf human/.style={gf box,draw=gfTeal,fill=gfTealFill},
  gf account/.style={gf box,draw=gfOchre,fill=gfOchreFill},
  gf flow/.style={
    -{Latex[length=4pt,width=3.3pt]},draw=gfInk,line width=0.75pt
  },
  gf access/.style={gf flow,dash pattern=on 2.4pt off 1.7pt},
  gf small/.style={
    font=\fontfamily{phv}\selectfont\fontsize{7}{8.5}\selectfont
  },
  gf heading/.style={
    font=\fontfamily{phv}\selectfont\fontsize{8}{9.5}\selectfont\bfseries,
    anchor=west
  }
}

